MLRS-PDS: A Meta-learning recommendation of dynamic ensemble selection pipelines

Dynamic Selection (DS), where base classifiers are chosen from a classifier's pool for each new instance at test time, has shown to be highly effective in pattern recognition. However, instability and redundancy in the classifier pools can impede computational efficiency and accuracy in dynamic ensemble selection. This paper introduces a meta-learning recommendation system (MLRS) to recommend the optimal pool generation scheme for DES methods tailored to individual datasets. The system employs a meta-model built from dataset meta-features to predict the most suitable pool generation scheme and DES method for a given dataset. Through an extensive experimental study encompassing 288 datasets, we demonstrate that this meta-learning recommendation system outperforms traditional fixed pool or DES method selection strategies, highlighting the efficacy of a meta-learning approach in refining DES method selection. The source code, datasets, and supplementary results can be found in this project's GitHub repository: https://github.com/Menelau/MLRS-PDS.

==> removed.tex <==
The whole process can be divided into six main steps, as described below: 

\textbf{Step (1) - Meta-features extraction}: This process begins with the extraction of meta-features, $\mathbf{x}' = \{ (m_{f}_{1}, \ldots, (m_{f}_{n} \}$ from each dataset under consideration. Hence, the output of this step is a meta-feature vector, \(\mathbf{x'}\), extracted for each dataset in the set of datasets.

\textbf{Step (2) - Generating sets of pools and DS methods}: In this step, a set of pools of classifiers, represented as \(\mathbb{P} = \{ P_{1}, \ldots, P_{K} \} \), is generated. These pools are then paired with the set of DS techniques, denoted as \(\mathbb{DS} = \{ DS_{1}, \ldots, DS_{W} \}\), creating comprehensive combinations for evaluation. Thus, given that $\mathbb{DS}$ and $\mathbb{P}$ correspond to all DS techniques and pool generation schemes considered in the recommendation system, respectively, a total of $\left | \mathbb{DS} \right | \times \left | \mathbb{P} \right |$ models are generated during this step.

\textbf{Step (3) - Assessment of DS Method Performance}: In this step, we assess the performance of DS methods when using the generated pools of classifiers as inputs by calculating its classification accuracy for the corresponding dataset. During this step, all combinations of pool generation and methods are evaluated and their corresponding accuracies are obtained to be used in the next stage while defining the meta-target.

\textbf{Step (4) - Meta-target determination}: In this step, the meta-target should be determined. The meta-target is defined as the combination that obtains the highest accuracy. The meta-learning recommendation system allows us to investigate three possible recommendation scenarios:

\begin{itemize}
    \item \textbf{Scenario I, MLRS-P:} recommend an optimal pool generation scheme. In this meta-learning scenario, the meta-target $y'= y'_{pool}$ is the pool generation scheme that obtained the higher classification performance when used as input for the predefined DS (PDS) method specified by the user. In this case, \mathbb{DS} consists of a single model that is the predefined DS.

    \item \textbf{Scenario II, MLRS-DS:} involves recommending the best DS method only. Here, the meta-target $y'= y'_{DS}$ is the DS method that exhibited the highest classification performance according to the predetermined pool generation scheme (PP). In this case, \mathbb{P} consists of a single pool that is the PP.

    \item \textbf{Scenario III, MLRS-PDS:} consists of recommending an optimal pair (Pool, DS) automatically. In this context, the meta-target represents the pair (Pool, DS) that delivered the best performance in comparison to other pairs across our study. Hence, in this scenario, the meta-target consists of a tuple $y'= (y'_{pool}, y'_{DS}$ and can be considered a multi-label meta-learning problem. In this scenario, both \mathbb{P} and \mathbb{DS} consists of multiple elements.

\end{itemize}

\textbf{Step (5) - Meta-dataset}: At the outset of this step, a meta-dataset, $MT$, is constructed by combining the meta-feature vector, \(\mathbf{x'}\), with their corresponding meta-target, \(y’\) extracted of all datasets in $\mathbb{T}$. 

\textbf{Step (6) - Meta-model training}: The meta-learning recommendation system trains a meta-model, $M_m$, using the meta-dataset, $MT$. Thus, the meta-model $M_m$ is trained to learn the relationship between the meta-features $\mathbf{x}'$ (i.e., dataset characteristics) and the meta-targets $y'$ to propose recommendations while used to suggest recommendations for new datasets. It is important to mention here that different meta-learning formulations (i.e., different scenarios) generate a different meta-classifier $M_m$ and are considered as a distinct meta-problem. These three scenarios are evaluated in the experimental study of this chapter in order to validate their impact on the system's performance.

To provide a thorough understanding of the datasets used in this study and the rationale behind their selection, we begin by introducing the problem and the methodology proposed by Macia \cite{macia2010landscape}.

The idyllic landscape dataset, comprising artificial datasets created via Evolutionary Multi-objective Optimization (EMO), spans a range of data complexities. It includes two sets: S1 for algorithm training, which is binary labeled, and S2 for testing, which is unlabeled. These datasets vary in complexity according to metrics proposed by Ho (2002) and others, aiming to evaluate and compare different learning algorithms' performance. Complexity measures used in dataset generation, such as feature dimensions and Fisher’s discriminant ratio, are detailed in Table \ref{tab:complexity-metrics}.

The article \cite{sun2019meta} presents a meta-transfer learning approach for few-shot learning, which addresses the challenge of learning from a few examples. The authors propose a meta-learning framework that transfers knowledge from pre-trained models to new tasks with few labeled examples. They evaluate their approach on several benchmark datasets and demonstrate its effectiveness in improving few-shot learning performance. The authors also compare their approach to state-of-the-art few-shot learning methods and show that it outperforms them. The results suggest that meta-transfer learning is a promising approach for few-shot learning tasks. Additionally, the authors show that their meta-transfer learning approach can be used to improve the performance of ensembles of few-shot learners. They propose a method for ranking the few-shot learners based on their performance on a validation set and use the ranked learners to construct an ensemble. The results demonstrate that their approach outperforms other ensemble methods on several benchmark datasets. The authors conclude that their meta-transfer learning approach, combined with ensemble learning and ranking, can significantly improve the performance of few-shot learning systems.

In the paper \cite{gemp2017automated}, the authors explore state-of-the-art meta-learning methodologies and identify the limitations and research challenges in addressing Data preprocessing that is a challenging task in machine learning applications, involving data cleaning, imputation, and feature normalization, dimensionality reduction, and data balancing. Meta-learning encodes datasets with informative statistics called meta-features, assuming that similar datasets in meta-feature space exhibit similar behavior when used with similar models. Also, in the paper \cite{zagatti2021metaprep}, the authors propose a meta-learning-based recommendation system for data preparation. The system suggests five ranked pipelines, catering to users with different levels of experience. The top-ranked pipeline improves the performance of an AutoML system and is comparable to a reinforcement-learning-based algorithm but significantly faster. The method is tested in a real-world application, demonstrating its benefits and limitations. Overall, this work addresses the need for automating data preparation in AutoML platforms using meta-learning, showing promising results. Furthermore, the article \cite{bilalli2016automated}, uses meta-learning for automated Data Pre-processing. The extensive evaluation conducted in this paper demonstrated that applying the recommended transformations enhances the final result of the algorithms for a wide range of datasets.

The paper \cite{garcia2018classifier}  explores the use of complexity measures to enhance understanding and differentiate the performance of different techniques, considering factors such as class overlap, data separability, and distribution. The study compares various regression models' effectiveness in predicting classifier accuracies for classification problems. The results show that these models can accurately predict accuracies and identify the best classifier, outperforming randomly chosen or fixed classifiers. Using data complexity measures, accurate meta-models are built to predict expected accuracies and select the best classifier among popular techniques like  Artificial Neural Networks (ANN), Support Vector Machines (SVM), Decision Tree (DT), and K-Nearest neighbors (kNN). Comparisons with baseline recommenders highlight the superior performance of meta-regressors Distance Weighted k-Nearest Neighbor (DWNN), Random Forests (RF), and Support Vector Regressors (SVR), with RF utilizing important complexity measures based on neighborhood information and structure.

This collective research underscores the pivotal role of meta-learning in refining machine learning processes, from enhancing data preparation to optimizing classifier selection.


\cite{feurer2015efficient} proposed a meta-learning approach for automated machine learning by combining ensemble methods and Bayesian optimization. The meta-learning applied in this method is performed for warm-starting the Bayesian optimization technique. Their approach involved training meta-models to predict the performance of different learning algorithms on new datasets and using them to construct ensembles that achieved state-of-the-art performance on various classification tasks.

The size of the pool is important for controlling computational complexity and performance. Determining the appropriate pool size depends on factors like the choice of base classifiers, the DS method used, and the problem characteristics. Traditionally, researchers set a pre-specified pool size due to the computational expense of evaluating different sizes. However, this may limit the DS method's performance. The article \cite{roy2016meta} proposed the prediction of the best size of a pool of classifiers for META-DES based on the classification complexity using the meta-learning method. This method builds a meta-regression model by extracting complexity measures and the best pool size of datasets. By using the meta-regression model, the prediction of the pool size for a given data is accessible. In the paper \cite{roy2016meta}, a meta-regression model that predicts a suitable pool size for DS algorithms based on the problem's intrinsic classification complexity is proposed. The prediction process in this article follows a meta-learning framework, involving training and application phases to obtain meta-examples and train a meta-regression learner for pool size prediction. In the application phase, the trained model is used to predict the best pool size for unseen datasets based on their meta-features. 

%In meta-learning, selecting appropriate meta-features from datasets is crucial. Early work by Todorovski (2000) used the zooming-ranking method for meta-feature selection, focusing on classical feature selection techniques. Kalousis (2001) also tackled meta-feature selection but limited their study to algorithm pairs, aligning with their meta-learning definition. Reif et al. (2014) evaluated various meta-feature categories to predict classification accuracies, applying an automatic selection method to the meta-features, although they provided limited method details and used a small dataset range. Smith et al. (2014) explored algorithm and hyperparameter recommendations using meta-learning, leveraging past performance data. They demonstrated the efficacy of their method against standard approaches like grid and random search, suggesting its potential in automating machine learning and enhancing accessibility for non-experts.

Souza et al. \cite{souza2017characterization} introduced a comprehensive overview of the Oracle model and its relevance in the literature, particularly in relation to DCS techniques. The study highlighted the challenges faced by DCS techniques in selecting the best classifier according to the Oracle model, resulting in noticeable differences in accuracy rates. To address this issue, an ensemble generation method was proposed, ensuring a 100\% Oracle accuracy rate in the training set. This incremental method generated binary classifiers by placing hyperplanes in the feature space, guaranteeing at least one competent classifier for each training instance. The method proved to be faster than traditional ensemble approaches and allowed for the automatic determination of the pool size based on the training data. Experimental results revealed a significant disparity between the theoretical limit and DCS techniques when pools were generated without Oracle information. Even with a 100\% Oracle accuracy rate, the average accuracy rate achieved by DCS techniques was approximately 85\%, indicating their struggle in selecting the most competent classifier. This discrepancy suggests that the Oracle model, despite its use in the literature, may not be the optimal guide for identifying a promising pool for DCS techniques, as these techniques rely on local data rather than global information provided by the Oracle model. 


A crucial factor in enhancing the performance of DS methods is the selection of an appropriate pool generation scheme to create a pool of classifiers as input for DS algorithms. This is of paramount importance because, in scenarios where there is no single local expert in the pool or the quantity of local experts for a given instance is low, the task of selecting an effective ensemble becomes either impossible or significantly challenging for a DS method. The selection of pool generation schemes for DS algorithms can be categorized into two main perspectives: global and local. It is observed that the majority of DS publications tend to employ global perspective pool generation schemes, while the utilization of local perspective schemes is relatively limited. An online pool generation method \cite{souza2019online} creates a local perspective pool of classifiers specifically for test samples in difficult regions of the feature space, considering the estimated classification difficulty of instances. By using classifiers generated locally, the DCS techniques can more effectively select the appropriate classifier for instances prone to misclassification. For query samples surrounded by easy instances, a simple nearest neighbors rule is employed. The method involves creating a local pool (LP) consisting of specialized classifiers. Each classifier is selected using a DCS technique from a local sub-pool that contains at least one competent classifier for each instance in the class overlap regions of the feature space. If the unknown instance's Region of Competence (RoC) is located in a difficult region, the LP is dynamically generated using neighboring instances and used to label the query sample. However, if the query instance is far from the class boundaries, no pool is generated, and a simple nearest neighbors rule is used to obtain the output label. This work presents a methodology specifically designed for Dynamic Classifier Selection (DCS) techniques, not Dynamic Ensemble Selection (DES) which are promising in this field. In addition, the authors did not explore the utilization of meta-learning in the article.


Monteiro et al. \cite{monteiro2021classifier} proposed a method that is a classifier pool generation approach guided by diversity estimated from data complexity and classifier decisions. The process starts by assessing the behavior of complexity measures on different subsamples of the dataset. Complexity measures that exhibit high variability across subsamples are selected for further pool adaptation. An evolutionary algorithm is then employed to optimize diversity in both the complexity space and the decision space. The proposed method focuses on creating a pool of classifiers by leveraging two types of diversity: complexity diversity and decision diversity. Complexity diversity involves training classifiers on dataset subsets that represent sub-problems with varying levels of complexity. Decision diversity aims to generate classifiers that make different types of errors. The authors hypothesize that both types of diversity can guide the pool generation process as an optimization problem, which is solved using a multi-objective genetic algorithm. The contribution of this work lies in two aspects. Firstly, a new method for pool generation is proposed, which trains classifiers on data subsets with different complexity levels. Secondly, the authors demonstrate the positive impact of this approach when combined with dynamic selection methods. This method has a global perspective on problems. 

The analysis operates on two fundamental hypotheses: the null hypothesis (\(\textbf{H}_0\)) and the alternative hypothesis (\(\textbf{H}_1\)). Rejecting \(\textbf{H}_0\) implies that the DS technique in question exhibits a statistically significant enhancement in performance compared to the baseline method. To apply this test accurately, it is imperative to calculate the critical value (\(n_c\)) through the formula presented in Equation \ref{nul}. This calculation determines the threshold for statistical significance between the control and compared techniques.

\begin{equation} 
 n_{c} = \frac{n_{exp}}{2} + z_{\alpha} \sqrt{\frac{n_{exp}}{2}}  \label{nul}
\end{equation}

where $n_{exp}$ is the total number of experiments, and $z_{\alpha}$  is the critical value of the standard normal distribution for a significance level of ${\alpha}$ = 0.05. In this study, with a total of 288 tests and a significance level of 0.05, the calculated critical value ($n_{c}$) is 164. Therefore, if the number of wins is greater than or equal to 164, the null hypothesis that the technique being tested is no better than the baseline can be rejected with a significance level ${\alpha}$ = 0.05 (i.e., a confidence level of 95\%) (\citerefs{demvsar2006statistical}).

Meta-learning has been extensively applied in data preparation and classifier selection, as highlighted in various studies \cite{zagatti2021metaprep, bilalli2016automated,reif2014automatic,smith2014recommending,garcia2018classifier}

Similar to the previous scenarios, three algorithms, including Random Forests (RF), K Nearest Neighbors (KNN), and Support Vector Machine (SVM), were initially considered as meta-models for the MLRS-PDS. To compare the performance of the proposed MLRS-PDS, the Jaccard similarity coefficient score is used since it is commonly used in multi-label classification problems (\citerefs{rinartha2017comparative}). 

In the field of machine learning, significant advancements have been made in data preprocessing and algorithm selection through meta-learning. Gemp et al. ~\cite{gemp2017automated} critically examined meta-learning methodologies, highlighting challenges in data preprocessing tasks like cleaning and normalization. Building on this, ~\cite{zagatti2021metaprep} introduced a meta-learning system that enhances AutoML system performance and speed in data preprocessing steps. Additionally, Bilalli et al. (2016) showcased that applying meta-learning in automated data preprocessing significantly improves algorithm outcomes across various datasets.

Complementing this, the article "Using meta-learning for multi-target regression" (\cite{aguiar2022using}) proposes a new meta-learning method for building ensembles of regression models for multiple targets. This approach utilizes meta-features for dataset description and meta-learning algorithms for optimal model selection in the ensemble. When compared to other methods across various datasets, this approach demonstrates superior performance, highlighting the crucial role of meta-features in the method's success. 

%Overall, this meta-learning recommendation approach offers a novel solution for optimizing DS methods. It takes into account the dataset characteristics (i.e., the problem to be solved) and the DS model or criteria used for selecting and combining classifiers. This contributes to advancing the field as it is the first research work to specifically model these two properties to optimize the whole system's performance.


\begin{comment}
The first contribution of this research is the analysis of global and local perspective pool generation schemes for DS algorithms. We aim to understand how these different approaches affect the performance of DS techniques when the generated pool of classifiers is used as input for these methods. Because the local and global pool generation schemes would be used in the design of a novel method. 

Up to this point, the literature has predominantly utilized global perspective pool generation schemes for DS methods \cite{ko2008dynamic, woods1997combination, cruz2015meta}, while techniques that explicitly leverage local information for pool generation, such as the Forest of Local Trees (FLT) \cite{armano2018building} and Locally independent classifiers (LIT) \cite{ross2020ensembles}, have not been considered in this context yet. Thus, we want to first analyze which is more suitable for the DS method among the global perspective pool generation schemes. Secondly, \textbf{we hypothesize that since the base classifiers selection mechanism in DS algorithms is based on local information, local pool generation schemes have the potential to enhance the performance of DS techniques}. It means while global pool generation schemes should not be ignored, local pool generation schemes should not be neglected as well. In addition to global pool generation schemes. So we want to know how much local pool generation scheme would be suitable for DS methods. 

In line with this contribution, our research questions are:  

\begin{itemize}
  \item RQ1: Do local pool generation schemes achieve better results when used for dynamic selection algorithms?
  \item RQ2: Does selecting the best pool of classifiers, \( C_{} \), depend on what dynamic selection is used ?
  \item RQ3: Does selecting the best DS method depend on what pool of classifiers, \( C_{} \), is used?
  \item RQ4: Is there a relationship between static ensemble and dynamic selection results?
  \item RQ5: Does selecting the best pool of classifiers, \( C_{} \), for dynamic selection methods depend on what dataset is used?
\end{itemize}
\end{comment}

%Seven dynamic selection algorithms were used in this research using DESlib version 0.3.5 as the DS library \cite{cruz2020deslib}. In order to obtain meaningful results and ensure a diverse set of models, we considered three DCS (Dynamic classifier selection) and four DES (Dynamic ensemble selection) methods. The following is a compilation of the names of the methods: Overall Local Accuracy (OLA) \cite{woods1997combination} and Modified Local Accuracy (MLA) \cite{smits2002multiple} as DCS and KNORA-E \cite{ko2008dynamic}, KNORA-U \cite{ko2008dynamic}, Meta-learning for dynamic ensemble selection (META-DES) \cite{cruz2015meta}, Multiclass Imbalance (DES-MI) \cite{garcia2018dynamic}, and Dynamic Ensemble Selection performance (DES-P) \cite{woloszynski2012measure}. All DS techniques are based on the K-Nearest Neighbors (KNN) method, with the region of competence size (K) set to 7, following~\cite{cruz2015meta}. For the META-DES algorithm, the competence of base classifiers is estimated using 5 output profiles, and its meta-classifier employs a Multinomial Naive Bayes~\cite{cruz2015metah}. 


Three algorithms, including Random Forests (RF), K Nearest Neighbors (KNN), and Support Vector Machine (SVM), evaluated as the meta-modal based on previous studies cite{bilalli2017predictive, khan2020literature}. \textcolor{red}{Since the RF with a maximum depth of 5 obtained be overall best results, we used this classifier to build the meta-model in our system.}

%To find which technique is more effective as a meta-model, $M_m$, in this scenario, multiple runs were conducted with different hyperparameter configurations. For K Nearest Neighbors, values of K ranging from 2 to 6 were tested, while for Random Forests, Max Depth values of 2 to 5 were tried. The hyperparameter chosen for the Support Vector Machine was gamma equal to 'scale' (i.e., $1 / (n\_features \times X.var())$) and the cost, $c=1$ (\citerefs{pedregosa2011scikit}). %The results of the runs and the corresponding hyperparameters are presented in Table \ref{result0}.

%The approach consists of three phases. In the first phase, it predicts which pool of classifiers is better suited for DS algorithms, considering data characteristics and selecting the pool that would provide the best performance. In the second phase, the approach predicts which DS method is appropriate for a given pool of classifiers based on the characteristics of a given dataset. This ensures that the selected DS method is the best fit for the specific pool of classifiers. In the third and final phase, the approach predicts the best combination of pool and DS methods for given input data. It works by first recommending which pool of classifiers is more suitable according to the dataset characteristics. Then, the information of the selected pool is added to condition the recommendation of the best DS model. Thus, it offers a novel solution for optimizing DS methods in fully automated meta-learning recommendation model for dynamic selection pipelines.


%While this study has provided valuable insights into automated recommendations for pool generation schemes and selecting a DS method for a given data, there remain several intriguing opportunities for future research and enhancements. Here are some future works in this area:


%This approach, empirically tested over 288 datasets, has shown superior performance compared to traditional methods of selecting pool classifiers and DS techniques. The findings of our study also show the effectiveness of dynamic selection hinges critically on the careful selection of the classifier pool, which must align with the unique characteristics of each dataset as well as the DS method employed. These results confirms the strong relationship between pool selection and dataset attributes, revealing that a one-size-fits-all approach falls short. Instead, our work emphasizes the necessity of a bespoke strategy in classifier selection, tailoring to the distinct demands of each specific dataset to optimize dynamic selection performance.

%The meta-learning recommendation system introduced in this project represents a significant advancement in the field of dynamic selection. By constructing a meta-model using meta-features and meta-targets, this system recommends an appropriate pool generation scheme for DS techniques, the best DS method, and an optimal pair of (DS, Pool) for a given dataset. 

%our system can adeptly recommends the most suitable pool generation scheme, identifies the best DS method, and determines the optimal (DS, Pool) pair for a given dataset. As such it can be employed in different use cases: 1) User has already a pretrained pool of classifiers an wants to improve the recognition performance by selecting the most adapted DS technique; 2) 

The empirical study conducted on 288 datasets with varying complexity level demonstrate that our approach outperforms traditional methods in selecting pool classifiers and Dynamic Selection (DS) techniques. The study highlights the importance of choosing a classifier pool that aligns with each dataset's unique characteristics and the specific DS method used, underlining the ineffectiveness of a generic approach. These findings advocate for a customized strategy in classifier selection to enhance dynamic selection effectiveness. It also demonstrate that training the pool of classifiers should not be neglected when employing DS methods in practice. Future work will involve in improving the meta-learning framework to also recommend the hyperparamters of the DS models and pool generation schemes involved as well as evaluate different alternatives for the meta-features extraction process.

%\end{itemize}


%To improve the performance and reduce the burden of finding the optimal solution through a costly optimization scheme, we propose a meta-learning recommendation system (MLRS) that can work in three scenarios: 1) recommend the best pool generation scheme according to the problems characteristics and a given DS model specified by the user; 2) recommend the best DS method given the problem characteristics a predefined pool generation scheme; 3) recommend the pair (DS, Pool) in a fully automated fashion just taking into account the problem characteristics. It works by first recommending which pool of classifiers is more suitable according to the dataset characteristics. Then, the information of the selected pool is added to condition the recommendation of the best DS model. Thus, it offers a novel solution for the performance of DS system in fully automated meta-learning recommendation model for dynamic selection pipelines.

%The main contribution of this work is the development of a meta-learning recommendation approach for Dynamic Selection (DS) methods. With the application of meta-learning, we extract meta-features from a given dataset and predict using a meta-model built during the training step. This meta-model is constructed from the meta-features extracted from training datasets and the best performance of various pools of classifiers used as input for DS algorithms.

\begin{comment}
Scenario I - Since the
RF with a maximum depth of 5 obtained be overall best results, we used this classifier to build
the meta-model in our system.

Scenario II - Based on this analysis we can conclude that the KNN with the k equal to 2 is the best approach
to be used as the meta-classifier for Scenario II (MLRS-DS)

Scenario III - It can be observed that the KNN with K equal to 2 obtains a
higher score when used as the meta-model

\begin{table}[H]
\centering
\caption{Hyper-parameters considered for machine learning and ensemble models.}
\resizebox{0.35\textwidth}{!}{%

		\begin{tabular}{ll}
			\hline
			\textbf{Scenario} & \textbf{Meta-learner configuration}
			\\ \hline
			\textbf{Scenario I} ($\lambda_{pool}$) & KNN\\ \hline

			\textbf{Scenario II} & RF \\ \hline
				
			\textbf{Scenario III} ($\lambda_{pool, DS}$) & RF \begin{tabular}[c]{@{}l@{}}bootstrap: [True, False]\\ max\_depth: [5,10, 20, 30, 40, 50]\\ max\_features: ['auto', 'sqrt', 'log2']\\ min\_samples\_leaf: [1, 2, 4]\\ min\_samples\_split: [2, 5, 10]\\ n\_estimators: [200, 400, 600, 800, 1000]\\  criterion: ['gini', 'entropy']\end{tabular} \\ \hline
   			
		\end{tabular}%
		}
	\label{tab:hyperparameter_grid-1}
\end{table}
\end{comment}

\begin{comment}
\begin{table}
\centering

\caption{Recommendation accuracy of the MLRS-P compared to the recommendation based on the majority and the average of all possible combinations. Each row corresponds to the results of the pool recommendation task according to a specific DS algorithm in question. The value inside parenthesis represents the number of datasets that the corresponding method recommended the best pool generation scheme}
\label{result1}
\small
\begin{tabular}{|l|l|l|l|}
\hline
Algorithm & MLRS-P (\# Datasets) & majority & Average \\
\hline
KNORA-E & 79.16(228) & 31.25(90) & 21.92(43) \\
META-DES & 71.87(207)& 31.25(90)  & 24.84(44.86) \\
KNORA-U & 70.13(202)& 36.11 (104)  & 25.04(48.29) \\
DES-MI & 78.12(225) & 38.19(110) & 22.26(42.86) \\
DES-P & 71.52(206)& 35.41(102)  & 25.24(45.29) \\
MLA & 66.66(192)& 26.38 (76)  & 24.65(48.14) \\
OLA & 62.84(181)& 48.26 (139)  & 20.83(42.71) \\  
\hline
\end{tabular}
\end{table}
\end{comment}

Additionally, our results reveal that relying on a single, seemingly optimal configuration, such as the RF model in this case, results in sub-optimal performance, achieving the best results in less than 50\% of cases.

In contrast,  the average performance of DS methods that use LIT, including (KNORA-E, LIT), (META-DES, LIT), (KNORA-U, LIT), (DES-MI, LIT), (DES-P, LIT), (MLA, LIT), (OLA, LIT) was 21.87\%, with the average number of wins among these combinations being 42.71. The majority


%Dynamic selection (DS) within MCS, characterized by selecting classifiers based on each specific instance, has gained prominence in multiple pattern recognition contexts such as imbalanced learning~\cite{cruz2019dynamic}, noisy data handling~\cite{walmsley2022investigation}, and concept drift~\cite{almeida2018adapting}, showcasing their wide-ranging impact.It aims to enhance classification accuracy by selecting the most competent classifiers from a pool, tailored to each instance at test time~\cite{cruz2018dynamic}. As such, they require a suitable pool of classifiers as input that is well suited to the classification problem in hand and covers the whole feature space, so that the DS method can single out the best ones~\cite{oliveira2017online}. 

%However, existing literature lacks specific guidance on selecting or training classifier pools optimized for dynamic selection (DS) algorithms with only few papers tackling this issue~\cite{souza2019online}. Furthermore, the generation process proposed in~\cite{souza2019online} works in an online scenario and is available for dynamic classifier selection techniques. While many DS studies rely on conventional pool generation schemes like Bagging \cite{breiman1996bagging}, Boosting \cite{freund1997decision}, and Random Forests \cite{rodrigues2023security}, these pool generation schemes were primarily tailored for static combinations and do not account for the local assumptions inherent in DS models, leading to uncertainty in generating experts to cover the entire feature space \cite{cruz2019fire, oliveira2017online}. Furthermore, the DS field has yet to address which pool generation scheme is best suited for DS methods. Most research in this area focuses on enhancing competence level estimation, ensemble selection, or region of competence definitions for better performance. This approach often assumes that pools created by traditional ensemble techniques like Bagging or Boosting are universally applicable across all classification problems, thereby overlooking the significant influence of the classifier pool's composition.

%However, there is a lack of specific guidance in the literature on how to select or train a pool of classifiers optimized for dynamic selection algorithms. The majority of DS publications use conventional pool generation schemes like Bagging \cite{breiman1996bagging}, Boosting \cite{freund1997decision} and Random Forests~\cite{rodrigues2023security}. Nevertheless, these methods were developed for static combination and are not based on the local assumption of DS models, having no guarantee that experts are generated to cover the whole feature space~\cite{cruz2019fire,oliveira2017online}. Furthermore, no previous study in DS addressed specifically the question on which is the best pool generation scheme to be used as input for DS methods. The majority of techniques from the DS literature focus on improving the competence level estimation and/or the ensemble selection steps, or improving region of competence definitions to improve performance. These, are assumes that the pool of classifiers generated with classical ensemble learning techniques such as Bagging or Boosting always provides a suitable pool of base models for any classification problem. Thus, neglecting the impact of the pool of classifiers used as input

%This study introduces Meta-learning for Imbalanced Re-gression (Meta-IR), a meta-learning recommendation system for addressing imbalanced regression tasks. Algorithms and techniques are recommended based on problem meta-features, serving as input to the meta-classifier. The meta-classifier suggests an optimal resampling strategy and learn-ing algorithm—a pipeline—customized to a new problem’smeta-features. For example, for a given dataset, it could recommend the Random Over-sampling strategy with the Decision Tree learning model

%The experimental analysis including 218 datasets, six learning models, six resampling strategies, and no resampling showed that Meta-IR outperforms the Random recommendation and Majority (always recommends the technique that appears most frequently in the meta-dataset) at the meta-level. At the base-level, comparing the performance achieved by the recommended learning models and resampling strategies, Meta-IR recommendations were better than Random, Majority and Auto-sklearn. Furthermore, statistical analysis revealed that the proposed method produces statistically significant results at this level. In conclusion, the Meta-IR approach demonstrated an advantage in terms of time efficiency, as it proved to be approximately 50 times faster than the Auto-sklearn.

%The meta-learning recommendation system (MLRS) can operate in three distinct scenarios for optimizing dynamic selection (DS) processes. In the first, MLRS-P, it is trained recommends a pool generation scheme assuming the user has already chosen a DS method, focusing on identifying the most suitable pool condition to that specific method. The second scenario, MLRS-DS, involves recommending a DS method when the user has a specific pool generation scheme in mind, guiding them to the DS method that best complements their chosen pool. Lastly, the third scenario, MLRS-PDS, offers a fully automated approach where the system recommends both a pool generation $P_o$ scheme and a DS, $DS_o$ method conditioned to the recommended pool. Hence, it consists of a chained recommendation procedure.



   % \item \textbf{Scenario II, MLRS-DS:} involves recommending the best DS method only. Here, the meta-target $y'= y'_{DS}$ is the DS method that exhibited the highest classification performance according to the predetermined pool generation scheme. In this case, \mathbb{P} consists of a single pool that is the predefined pool generation scheme, and the meta-classifier $\lamndba_{DS}$ is trained specifically to make recommendations for it.

   % \item \textbf{Scenario III, MLRS-PDS:} consists of recommending an optimal pair (Pool, DS). In this context, the meta-target represents the tuple $(y'_{pool}, y'_{DS})$ that delivered the best performance in comparison to other configurations across our study. Hence, this scenario consists of a multi-label meta-learning recommendation problem. As such, the classifier chain method was considered to train the meta-classifier for this multi-label recommendation task. The order of prediction considered for this chained classification is pool first, then DS method. As this scenario consists on a fully automated fashion considering all possible configurations, both \mathbb{P} and \mathbb{DS} consists of multiple elements to generate the meta training data $MT$. 

   %Garcia et al.\cite{garcia2018classifier} explored the use of complexity measures in meta-learning to differentiate classifier performance effectively. Their study demonstrated that regression models like ANNs, SVMs, DTs, and kNNs could accurately predict expected classifier performances using meta-regressors.


==> supplementary_material.tex <==
\section{Meta-features}

Below is a brief description of each category:

\begin{itemize}
    \item \textbf{Statistical}: There are standard statistical measures to describe the numerical properties of data distribution (\citerefs{brazdil2008metalearning}). This category for extracting statistical meta-features from datasets covers a range of statistical computations, including computing correlations, covariances, median, minimum, and maximum values, and various other statistical measures for each attribute. 
    
    \item \textbf{Information-theoretic}: It encompasses a diverse set of measures used to analyze datasets' characteristics. They include the assessment of class label and attribute entropy, the quantification of relationships between variables, the evaluation of signal-to-noise ratios, and the estimation of effective attributes (\citerefs{brazdil2008metalearning}).
    
    \item \textbf{Model-based}: meta-features that are designed to capture characteristics of machine learning models, specifically Decision Tree (DT) models, induced from a dataset. These meta-features encompass specific properties, including depth, shape, and size, which can be indicative of the complexity and structure of the dataset. (\citerefs{pavel2002decision}).
    
    \item \textbf{Landmarking}: Performance of simple and efficient learning algorithms such as DEcision trees (DT) and K Nearest neighbors (KNN). The meta-features, $m_{f}$, collected in this category include relative and subsampling performances (\citerefs{reif2014automatic, smith2009cross, rivolli2018characterizing}, soares2001sampling).
    
    \item \textbf{Clustering-based}: This meta-feature collects information regarding both correlation and dissimilarity. The Correlation Measure quantifies the statistical relationships between pairs of instances in the dataset. The stronger similarity in attribute behaviors among instances results in a higher correlation. The Dissimilarity Measure is based on the Euclidean distance between instances, representing the distance between data points in the dataset (\citerefs{pimentel2019new}).
    
    \item \textbf{Concept}: Estimate the variability of class labels among examples and the example's density. 
    (\citerefs{rivolli2018characterizing}). Methods for extracting meta-features related to the Concept group from datasets cover computations such as cohesiveness, concept variation, improved concept variation, and weighted distance between examples of the same classes as well as different classes. Hence, they are measures to define whether a feature space is highly irregular (several small groups of samples belonging to the same class) or more uniform in which large regions of samples share the same class labels.
    
    \item \textbf{Itemset}: Compute the correlation between binary attributes (\citerefs{song2012automatic}).
    
    \item \textbf{Complexity}: Estimate the difficulty in separating the data points into their expected classes (\citerefs{lorena2019complex}). The extraction of meta-features related to dataset complexity involves various methods, covering computations such as entropy, imbalance ratio, clustering coefficient, network density, Fisher's discriminant ratios, hub scores, and a range of other complexity measures.
\end{itemize}

The list describing all meta-features considered in this work is presented in the Tables below:

\begin{table}[H]
\centering
\begin{minipage}{0.9\linewidth}
\caption{Meta-features present in the meta-dataset}
\label{mfff}
\scalebox{0.7}{
\begin{tabular}{|l|l|l|l|}
\hline
  & Meta feature & Group & Description \\
\hline

1  &  attr\_to\_inst & general & Compute the ratio between the number of attributes. \\

2  &  cat\_to\_num & general & Compute the ratio between the number of categoric and numeric features. \\
 
3  &  freq\_class & general & Compute the relative frequency of each distinct class. \\
% 3  &  freq\_class\_sd & general & Compute the standard deviation of the relative frequency of each distinct class. \\
 
4  &  inst\_to\_attr & general & Compute the ratio between the number of instances and attributes. \\
 
5  &  nr\_attr & general & Compute the total number of attributes. \\
 
6  &  nr\_bin & general & Compute the number of binary attributes. \\
 
7  &  nr\_cat & general & Compute the number of categorical attributes. \\
 
8  &  nr\_class & general & Compute the number of distinct classes. \\
 
9  &  nr\_inst & general & Compute the number of instances (rows) in the dataset. \\
 
10  &  nr\_num & general & Compute the number of numeric features. \\
 
11  &  num\_to\_cat & general & Compute the number of numerical and categorical features. \\
 
12  &  precompute\_general\_class & general & Precompute distinct classes and its frequencies from y. \\
 % nadasht 12
13  &  can\_cor & Statistical & Compute the canonical correlations of data. \\

% 13  &  can\_cor\_sd & Statistical & Compute the standard deviation of the canonical correlations of data. \\
 
14  &  cor & Statistical & Compute the absolute value of the correlation of distinct dataset column pairs. \\

% 14  &  cor\_sd & Statistical & Compute the standard deviation of the absolute value of the correlation of distinct dataset column pairs. \\
 
15  &  cov & Statistical & Compute the absolute value of the covariance of distinct dataset attribute pairs. \\
 
16  &  eigenvalues & Statistical & Compute the eigenvalues of covariance matrix from dataset. \\
 
17  &  g\_mean & Statistical & Compute the geometric mean of each attribute. \\
 
18  &  gravity & Statistical & Compute the distance between minority and majority classes center of mass. \\
 
19  &  h\_mean & Statistical & Compute the harmonic mean of each attribute. \\
 
20  &  iq\_rang & Statistical & Compute the interquartile range (IQR) of each attribute. \\
 
21  &  kurtosis & Statistical & Compute the kurtosis of each attribute. \\
 
22  &  lh\_trace & Statistical & Compute the Lawley-Hotelling trace. \\
 
23  &  mad & Statistical & Compute the Median Absolute Deviation (MAD) adjusted by a factor. \\
 
24  &  max & Statistical & Compute the maximum value from each attribute. \\
 
25  &  mean & Statistical & Compute the mean value of each attribute. \\
 
26  &  median & Statistical & Compute the median value from each attribute. \\
 
27  &  min & Statistical & Compute the minimum value from each attribute. \\
 
28  &  nr\_cor\_attr & Statistical & Compute the number of distinct highly correlated pairs of attributes. \\
 
29  &  nr\_disc & Statistical & Compute the number of canonical correlations between each attribute and class. \\
 
30  &  nr\_norm & Statistical & Compute the number of attributes normally distributed based in a given method. \\
 
31  &  nr\_outliers & Statistical & Compute the number of attributes with at least one outlier value. \\
 
32  &  p\_trace & Statistical & Compute the Pillai's trace. \\
 
33  &  range & Statistical & Compute the range (max-min) of each attribute. \\
 
34  &  roy\_root & Statistical & Compute the Roy's largest root. \\
 
35  &  sd & Statistical & Compute the standard deviation of each attribute. \\
 
36  &  sd\_ratio & Statistical & Compute a statistical test for homogeneity of covariances. \\
 
37  &  skewness & Statistical & Compute the skewness for each attribute. \\
 
38  &  sparsity & Statistical & Compute (possibly normalized) sparsity metric for each attribute. \\
 
39  &  t\_mean & Statistical & Compute the trimmed mean of each attribute. \\
 
40  &  var & Statistical & Compute the variance of each attribute. \\
\hline
\end{tabular}}
\end{minipage}
\end{table}


\begin{table}[H]
\centering
\begin{minipage}{0.9\linewidth}
\caption{Meta-features present in the meta-dataset}
\label{mfff}
\scalebox{0.57}{
\begin{tabular}{|l|l|l|l|}
\hline
  & Meta feature & Group & Description \\
\hline
41  &  w\_lambda & Statistical & Compute the Wilks' Lambda value. \\
 
42  &  precompute\_can\_cors & Statistical & Precompute canonical correlations and its eigenvalues. \\

43  &  precompute\_statistical\_class & Statistical & Precompute distinct classes and its abs. \\

44  &  precompute\_statistical\_cor\_cov & Statistical & Precomputes the correlation and covariance matrix of numerical data. \\

45  &  attr\_conc & Information theory & Compute concentration coef. \\

46  &  attr\_ent & Information theory & Compute Shannon's entropy for each predictive attribute. \\

47  &  class\_conc & Information theory & Compute concentration coefficient between each attribute and class. \\

48  &  class\_ent & Information theory & Compute target attribute Shannon's entropy. \\

49  &  eq\_num\_attr & Information theory & Compute the number of attributes equivalent for a predictive task. \\

50  &  joint\_ent & Information theory & Compute the joint entropy between each attribute and class. \\

51  &  mut\_inf & Information theory & Compute the mutual information between each attribute and target. \\

52  &  ns\_ratio & Information theory & Compute the noisiness of attributes. \\

53  &  precompute\_class\_freq & Information theory & Precompute each distinct class (absolute) frequencies. \\

54  &  precompute\_entropy & Information theory & Precompute various values related to Shannon's Entropy. \\

55  &  extract\_table & Model-based & Bookkeep some information table from the t\_model into an array. \\

56  &  leaves & Model-based & Compute the number of leaf nodes in the DT model. \\

57  &  leaves\_branch & Model-based & Compute the size of branches in the DT model. \\

58  &  leaves\_corrob & Model-based & Compute the leaves corroboration of the DT model. \\

59  &  leaves\_homo & Model-based & Compute the DT model Homogeneity for every leaf node. \\

60  &  leaves\_per\_class & Model-based & Compute the proportion of leaves per class in DT model. \\

61  &  nodes & Model-based & Compute the number of non-leaf nodes in DT model. \\

62  &  nodes\_per\_attr & Model-based & Compute the ratio of nodes per number of attributes in DT model. \\

63  &  nodes\_per\_inst & Model-based & Compute the ratio of non-leaf nodes per number of instances in DT model. \\

64  &  nodes\_per\_level & Model-based & Compute the ratio of number of nodes per tree level in DT model. \\

65  &  nodes\_repeated & Model-based & Compute the number of repeated nodes in DT model. \\

66  &  tree\_depth & Model-based & Compute the depth of every node in the DT model. \\

67  &  tree\_imbalance & Model-based & Compute the tree imbalance for each leaf node. \\

68  &  tree\_shape & Model-based & Compute the tree shape for every leaf node. \\

69  &  var\_importance & Model-based & Compute the features importance of the DT model for each attribute. \\

70  &  precompute\_model\_based\_class & Model-based & Precompute the DT Model and some information related to it. \\

71  &  best\_node & Landmarking & Performance of the best single decision tree node. \\

72  &  elite\_nn & Landmarking & Performance of Elite Nearest Neighbor. \\

73  &  linear\_discr & Landmarking & Performance of the Linear Discriminant classifier. \\

74  &  naive\_bayes & Landmarking & Performance of the Naive Bayes classifier. \\

75  &  one\_nn & Landmarking & Performance of the 1-Nearest Neighbor classifier. \\

76  &  random\_node & Landmarking & Performance of the single DT node model induced by a random attribute. \\

77  &  worst\_node & Landmarking & Performance of the single DT node model induced by the worst informative attribute. \\

78  &  precompute\_landmarking\_kfolds & Landmarking & Precompute k-fold cross-validation related values. \\

79  &  precompute\_landmarking\_sample & Landmarking & Precompute subsampling landmarking subsample indices. \\

80  &  group\_mtf\_by\_summary & Relative Landmarking & Group meta features by its correspondent summary method. \\

\hline
\end{tabular}}
\end{minipage}
\end{table}






\begin{table}[H]
\centering
\begin{minipage}{0.9\linewidth}
\caption{Meta-features present in the meta-dataset}
\label{mfff}
\scalebox{0.57}{
\begin{tabular}{|l|l|l|l|}
\hline
  & Meta feature & Group & Description \\
\hline
81  &  postprocess\_landmarking\_relative & Relative Landmarking & Generate Relative Landmarking from Landmarking metafeatures. \\

82  &  ch & Clustering & Compute the Calinski and Harabasz index. \\

83  &  int & Clustering & Compute the INT index. \\

84  &  nre & Clustering & Compute the normalized relative entropy. \\

85  &  pb & Clustering & Compute the Pearson correlation between class matching and instance distances. \\

86  &  sc & Clustering & Compute the number of clusters with sizes smaller than a given size. \\

87  &  sil & Clustering & Compute the mean silhouette value. \\

88  &  vdb & Clustering & Compute the Davies and Bouldin Index. \\

89  &  vdu & Clustering & Compute the Dunn Index. \\

90  &  precompute\_class\_representatives & Clustering & Precomputations related to cluster representative instances. \\

91  &  precompute\_clustering\_class & Clustering & Precompute distinct classes and its frequencies from y. \\

92  &  precompute\_group\_distances & Clustering & Precompute distance metrics between instances. \\

93  &  precompute\_nearest\_neighbors & Clustering & Precompute the n\_neighbors Nearest Neighbors of every instance. \\

94  &  cohesiveness & Concept & Improved weighted distance that captures how dense or sparse is the example distribution. \\

95  &  conceptvar & Concept & Compute the concept variation that estimates the variability of class labels among examples. \\

96  &  impconceptvar & Concept & Compute the improved concept variation that estimates the variability of class labels among examples. \\

97  &  wg\_dist & Concept & Compute the weighted distance and that captures how dense or sparse is the example distribution. \\

98  &  precompute\_concept\_dist & Concept & Precompute some useful things to support complexity measures. \\

99  &  one\_itemset & Itemset & Compute the one itemset meta-feature. \\

100  &  two\_itemset & Itemset & Compute the two itemset meta-feature. \\

101  &  precompute\_binary\_matrix & Itemset & Precompute the binary representation of attributes. \\

102  &  c1 & Complexity & Compute the entropy of class proportions. \\

103  &  c2 & Complexity & Compute the imbalance ratio. \\

104  &  cls\_coef & Complexity & Clustering coefficient. \\

105  &  density & Complexity & Average density of the network. \\

106  &  f1 & Complexity & Maximum Fisher's discriminant ratio. \\

107  &  f1v & Complexity & Directional-vector maximum Fisher's discriminant ratio. \\

108  &  f2 & Complexity & Volume of the overlapping region. \\

109  &  f3 & Complexity & Compute feature maximum individual efficiency. \\

110  &  f4 & Complexity & Compute the collective feature efficiency. \\

111  &  hubs & Complexity & Hub score. \\

112  &  l1 & Complexity & Sum of error distance by linear programming. \\

113  &  l2 & Complexity & Compute the OVO subsets error rate of a linear classifier. \\

114  &  l3 & Complexity & Non-Linearity of a linear classifier. \\

115  &  lsc & Complexity & Local set average cardinality. \\

116  &  n1 & Complexity & Compute the fraction of borderline points. \\

117  &  n2 & Complexity & Ratio of intra and extra class nearest neighbor distance. \\

118  &  n3 & Complexity & Error rate of the nearest neighbor classifier. \\

119  &  n4 & Complexity & Compute the non-linearity of the k-NN Classifier. \\

120  &  t1 & Complexity & Fraction of hyperspheres covering data. \\

\hline
\end{tabular}}
\end{minipage}
\end{table}

\begin{table}[H]
\centering
\begin{minipage}{0.9\linewidth}
\caption{Meta-features present in the meta-dataset}
\label{mfff}
\scalebox{0.7}{
\begin{tabular}{|l|l|l|l|}
\hline
  & Meta feature & Group & Description \\
\hline
121  &  t2 & Complexity & Compute the average number of features per dimension. \\

122  &  t3 & Complexity & Compute the average number of PCA dimensions per point. \\

123  &  t4 & Complexity & Compute the ratio of the PCA dimension to the original dimension. \\

124  &  precompute\_adjacency\_graph & Complexity & Calculate values associated with the nearest neighboring instances. \\

125  &  precompute\_complexity & Complexity & Precompute some useful things to support feature-based measures. \\

126  &  precompute\_complexity\_svm & Complexity & Init a Support Vector Classifier pipeline (with data standardization.) \\

127  &  precompute\_nearest\_enemy & Complexity & Precompute instances nearest enemy related values. \\

128  &  precompute\_norm\_dist\_mat & Complexity & Precompute normalized n and pairwise distance among instances. \\

129  &  precompute\_pca\_tx & Complexity & Precompute PCA to support dimensionality measures. \\

\hline
\end{tabular}}
\end{minipage}
\end{table}







